Certifiably Correct Range-Aided SLAM

We present the first algorithm to efficiently compute certifiably optimal solutions to range-aided simultaneous localization and mapping (RA-SLAM) problems. Robotic navigation systems increasingly incorporate point-to-point ranging sensors, leading to state estimation problems in the form of RA-SLAM. However, the RA-SLAM problem is significantly more difficult to solve than traditional pose-graph SLAM: ranging sensor models introduce non-convexity and single range measurements do not uniquely determine the transform between the involved sensors. As a result, RA-SLAM inference is sensitive to initial estimates yet lacks reliable initialization techniques. Our approach, certifiably correct RA-SLAM (CORA), leverages a novel quadratically constrained quadratic programming (QCQP) formulation of RA-SLAM to relax the RA-SLAM problem to a semidefinite program (SDP). CORA solves the SDP efficiently using the Riemannian Staircase methodology; the SDP solution provides both (i) a lower bound on the RA-SLAM problem's optimal value, and (ii) an approximate solution of the RA-SLAM problem, which can be subsequently refined using local optimization. CORA applies to problems with arbitrary pose-pose, pose-landmark, and ranging measurements and, due to using convex relaxation, is insensitive to initialization. We evaluate CORA on several real-world problems. In contrast to state-of-the-art approaches, CORA is able to obtain high-quality solutions on all problems despite being initialized with random values. Additionally, we study the tightness of the SDP relaxation with respect to important problem parameters: the number of (i) robots, (ii) landmarks, and (iii) range measurements. These experiments demonstrate that the SDP relaxation is often tight and reveal relationships between graph connectivity and the tightness of the SDP relaxation.

==> sections/3a_related_work_summaries.tex <==
\newpage

\subsection{Certificates}

%% point cloud / geometric registration
\subsubsection*{Geometric Registration}
\begin{itemize}
      \item \citet{iglesias20cvpr} - formulates point-set registration as QCQP
            (rotation search) and uses duality with a PSD-ness test to provide
            certificates. Evaluates how the certificates perform w.r.t. missing
            data and distribution of points. Show how to compute Lagrange
            multipliers from candidate solution and how to certify without
            solving any SDPs
      \item \citet{yang20tro} - TEASER: uses Lagrangian Duality and
            Douglas-Rachford splitting to find certificate matrix at
            intersection of PSD cone and an affine subspace, this must be done
            because the LICQ is not satisfied. Instead of using SDP solution for
            rotation search also proposes GNC as an alternative.
\end{itemize}

%% imaging
\subsubsection*{Multi-View Geometry}
\begin{itemize}
      \item \citet{garcia-salguero21ivc} - uses stationarity condition, I think a
            specific instance of the WAFR 2020 work that uses a rank-1 relaxation
      \item \citet{garcia-salguero21siamjis} - provide a simpler sufficient
            condition that guarantees that the solution is optimal. The intuitive idea
            is to define a region of solutions for which the positive semidefiniteness
            of the Hessian is guaranteed without computing explicitly its eigenvalues or
            the vector. Lots of pretty math, very complicated and bespoke to the problem
            at hand. However, the idea may generalize well.
      \item \citet{garcia-salguero22cviu} - primal dual solver for 2-view
            triangulation and very efficient optimality certification (linear solve +
            PSD-ness check). we derive a sufficient (but not necessary) optimality
            condition that allows us to certify optimality in less than one microsecond
      \item \citet{hartley13bijcv} - very cool, uses a PSD-ness test to check if
            the cost is convex over the domain, thus certifying any local optimum
      \item \cite{olsson09cvpr} - sufficient condition for optimality based on
            convexity over the problem domain. Also provides a BnB approach for global
            optimality when can't certify local solution, is a precursor to \citet{hartley13bijcv}
\end{itemize}

%% SLAM and localization
\subsubsection*{SLAM and Localization}
\begin{itemize}
      \item \citet{briales17ral} - like SE-Sync but optimizing over SE(d) instead of SO(d)
      \item \citet{briales16iros} - uses Lagrangian duality condition to have a
            semi-rigorous closed-form certification scheme for PGO, basically uses the
            KKT condition without recognizing it
      \item \citet{carlone15iros} - closed form certification of solution, shows
            how to recover solution from dual solution
      \item \citet{fan20tro} - SE-Sync for the 2D case with complex number representation
      \item \citet{dumbgen22ral} - range only localization, vectorized QCQP
            formulation, cool efficient certificate computation based on KKT conditions
            \important
      \item \citet{halsted22arxiv} - VERY similar QCQP approach, Riemannian opt
            over oblique manifold (equivalent to ours), certification based on dual
            solution, uses dual solution to determine starting point for primal
            point (solves dual problem)
      \item \citet{holmes22arxiv} - just the SE-Sync certification but with landmarks drawn out
      \item \citet{rosen19ijrr} - SE-Sync
\end{itemize}

%% General Optimization
\subsubsection*{Misc.}
\begin{itemize}
      \item \citet{zheng12globaloptimization} - a posteriori condition for zero
            duality gap, obtained by solving dual of Shor's relaxation
      \item \citet{li12optimizationtheory} - provides N+S condition for
            optimality of equality constrained bivalent QCQPs \important
      \item \citet{boumal15arxiv,boumal16neurips} - cover main optimality proofs
            of SE-Sync, some interesting stuff about only allowing for relative
            measurements  (e.g., no GPS or pinning poses)
      \item \citet{jeyakumar07mathprog} - same optimality criteria as in WAFR
            2020, just different QCQP formulation (vectorized) and does not admit a
            algorithm for certification \important
\end{itemize}
\newpage

\subsection{SDP-based approaches}
\subsubsection*{Geometric Registration}
\begin{itemize}
      \item \citet{briales17cvpr} - focuses on point cloud registration, uses
            Lagrangian duality and solves dual problem of fixed size to obtain
            globally optimal solution
      \item \citet{olsson08icpr} - formulate registration problem as QCQP and solve Lagrange dual SDP
      \item \citet{khoo16tip} - SDP relaxation of MI-NLP formulation of point
            cloud registration, simultaneous pose and correspondence problem
      \item \citet{yang19rss} - original TEASER paper, solve robust point cloud
            registration with SDP. a polynomial-time solution for each subproblem: scale
            and (component-wise) translation estimation can be solved exactly via an
            adaptive voting scheme, while rotation estimation can be relaxed to a
            semidefinite program. Certified if returns a rank-3 solution
      \item \citet{peng22techreport} - defines conditions under which a specific
            SDR is tight for the rotation search problem
      \item \citet{yang20neurips} - shows how to relax TLS to SOS optimization,
            with empirical tightness at lowest rank. Efficient certification scheme
            using Douglas-Rachford Splitting for the SOS dual problem
\end{itemize}
\subsubsection*{Multi-View Geometry}
\begin{itemize}
      \item \citet{aholt12lncs} - KKT conditions, SDP relaxation, multi-view
            imaging, appears to be application of same KKT condition rules we use
            \important
      \item \citet{briales18cvpr} - used Shor's relaxation for globally optimal
            relative pose estimation w/ cameras. Certified by checking primal
            feasibility of relaxed solution.
      \item \citet{garcia-salguero22jmiv} - solves a small scale SDP to solve a
            relaxed version of the problem, certified by checking tightness (if all
            constraints are satisfied), tackles the resolution of the Relative Pose
            problem with optimality guarantees by stating it as an optimization
            problem over the set of essential matrices that minimizes the squared
            epipolar error. We relax this non-convex problem with its Shor's
            relaxation, a convex program that can be solved by off-the-shelf tools.
            Uses redundant constraints to tighten the SDP relaxation.
      \item \citet{zhao20tpami} - SDR of a QCQP for essential matrix estimation.
\end{itemize}
\subsubsection*{SLAM and Localization}
\begin{itemize}
      \item \citet{carlone15bicra} - solves dual problem to get a tight lower
            bound for certification of 2D SLAM problems
      \item \citet{carlone16tro} - solves dual problem for planar PGO to get
            globally optimal solution, certifies optimality
            % \item \citet{wang22arxiv} - just uses SDR of a MIQCQP to obtain solution, certification is based on dual of SDR
      \item \citet{giamou19ral} - formulates the calibration problem as rotation
            averaging and solves a vectorized QCQP formulation via Lagrangian duality
\end{itemize}
\subsubsection*{Misc.}
\begin{itemize}
      \item \citet{barfoot22arxiv} - general least-squares fitting, a simplified
            example for the techniques used in TEASER \important
      \item \citet{bao11mathprog} - overview of SDP relaxations of QCQP problems
      \item \citet{nesterov00siam} - Some interesting details and examples on
            SDP relaxations of QCQPs. Has specific examples of when strong duality
            holds for QCQPs and some tricks for strengthening the dual relaxations via
            redundant constraints. Strong duality holds for orthonormal constraint
\end{itemize}
\newpage

\subsection{Polynomial Optimization}
\subsubsection*{Multi-View Geometry}
\begin{itemize}
      \item \citet{kahl07ijcv} - polynomial optimization applied to CV problems.
            The technique is applied to a number of classical vision problems:
            triangulation, camera pose, homography estimation and last, but not
            least, epipolar geometry estimation. I don't think this guarantees
            global optimality!
      \item \citet{mirzaei11iccv} - estimates vanishing points via polynomial
            systems, \Grobner~basis things
      \item \citet{mirzaei11icra} - Specifically, the optimality conditions of the
            least-squares problem form a system of polynomial equations, which we
            efficiently solve through the eigendecomposition of a so-called
            multiplication matrix. relaxes the problem and then exactly solves
            relaxation via Eigendecomposition.
      \item \citet{stewenius05iccv} - polynomial system, \Grobner~basis,
            algebraic geometry (similar to the range-only stuff from Stergios
            Roumeliotis)
\end{itemize}

%% SLAM and localization
\subsubsection*{SLAM and Localization}
\begin{itemize}
      \item \citet{trawny10icra} - \Grobner basis to solve relative position
            problem from ranges
\end{itemize}
\newpage

\subsection{Exhaustive Search Approaches}

%% point cloud / geometric registration
\subsubsection*{Geometric Registration}
\begin{itemize}
      \item \citet{ask13cvpr} - Low-dimensional approach for TLS in image
            registration, globally optimal by exhaustive search, uses clever tricks to
            reduce the number of scenarios evaluated
      \item \citet{bazin13lncs} - BnB solver to find the largest inlier set for rotation search
      \item \citet{olsson09tpami} - BnB to solve registration problems, use convex
            underestimators to get lower bounds
      \item \citet{izatt20isrr} - linear approximation of SO(d) and representation
            of point cloud alignment as mesh alignment to perform mixed integer linear
            (quadratic?) programming
      \item \citet{yang16tpami} - BnB for point cloud registration
\end{itemize}

%% imaging
\subsubsection*{Multi-View Geometry}
\begin{itemize}
      \item \citet{bazin14eccv} - BnB solver for focal length and orientation of
            camera for image relative pose search - extends 2013 LNCS work with
            application
      \item \citet{campbell17iccv} = bnb solver for correspondence-free 6-DOF
            relative camera pose estimation
      \item \citet{fredriksson16cvpr} - epipolar geometry and the correspondences
            using BnB
      \item \citet{hartley09ijcv} - BnB search to estimate essential matrix
      \item \citet{kneip13iccv} - global opt for frame-to-frame rotation
            estimation via BnB, also provides some eigenvalue bounds via perturbation
            theory
      \item \cite{lu07lncs} - BnB approach that uses LP solves for L2 triangulation
\end{itemize}
\newpage


==> sections/7a2_marine_experiments.tex <==
\subsubsection{Marine Experiments}
\label{sec:marine-experiments}

The marine experiments were conducted with the platforms described in
\cref{fig:marine-equipment} over a 250 meter by 100 meter river section. This
system was intended as a heterogeneous platform to investigate how agents with
high-accuracy navigation (\eg GPS or high-cost inertial navigation) could
enhance a low-accuracy navigation system. In this experiment the landmark (yellow
Jetyak) localizes via GPS fixes at 1 Hz, as proxy for high-accuracy navigation
system. In contrast, the Low-Nav craft (blue-white watercraft) obtains odometry
by combining heading estimates from a Sparton AHRS-M2 attitude heading reference
system with a constant-velocity assumption. The landmark effectively acts as a
moving landmark, with a GPS prior on its location and intermittent range
measurements to the Low-Nav Craft.

Inter-agent acoustic ranging used two Micromodem-2 systems
\cite{Gallimore10oceans}. Ground-truth vehicle positions were obtained from GPS
receivers mounted on each vehicle. The assumed constant velocity was obtained
from the average velocity over 10 hand-timed point-to-point 100 meter traverses.

Our estimation problem considers the GPS measurements of the landmark position,
inter-agent acoustic ranges, and the constant-velocity odometry. We jointly
estimate the pose of the Low-Nav craft and the positions of the landmark. Low-Nav
poses are taken at 1 Hz frequency while landmark positions are only considered
when new range measurements occur.

We present the estimated trajectories in \cref{fig:marine-trajectories} and the
associated error statistics in \cref{fig:traj-errors-bar-plot}.

\MarineExperimentalEquipmentFigure


==> sections/9c_preconditioner_and_saddle_escape.tex <==
\section{Riemannian Trust Region Preconditioning}
\label{sec:preconditioner}
\def \matP{\mat{P}}
\def \linearProblem{\matA x = b}
\def \preconditionedLinearProblem{\matP^{-1} \matA x = \matP^{-1} b}

We provide a brief overview of preconditioning and describe a
preconditioner {designed specifically for the Riemannian Trust Region (RTR)
optimizer \cite{absil07fcm} used in CORA.}

The convergence of conjugate gradients to solve the problem $\linearProblem$ is
highly dependent on the condition number $\kappa (\matA) \triangleq
    \frac{\lambda_{max}(A)}{\lambda_{min}(A)}$, as defined as the ratio of the largest
eigenvalue to the smallest eigenvalue of $\matA$
\cite[Section 10.3]{Golub96book}. The convergence can be improved by
preconditioning the problem with a matrix $\matP$ such that $\kappa(\matP^{-1}
    \matA) \ll \kappa(\matA)$. The (equivalent) preconditioned problem is then
$\preconditionedLinearProblem$.

The optimal preconditioner $\matP$ is the inverse of the matrix $\matA$, however
computing the exact inverse is equivalent to solving the original problem.
Thus, approximate preconditioners, which can be computed efficiently, are used
in practice; preconditioning strategies trade off the accuracy of the
preconditioner with the computational cost of computing the preconditioner.
Several common preconditioning strategies are the Jacobi preconditioner and its
block variant, the incomplete Cholesky preconditioner, and the regularized
incomplete Cholesky preconditioner \cite[Chapter 10]{saad2003iterative}.

{As outlined in \cref{sec:riemannian-staircase}, CORA uses the Riemannian
Trust Region (RTR) optimizer to solve the RA-SLAM problem. The RTR
optimizer solves a sequence of trust-region subproblems via truncated conjugate
gradients, which is where the preconditioner is applied. Critically, each
subproblem is a
}

\subsection*{Block-Diagonal Cholesky Preconditioner}

Whereas these preconditioners are designed for general systems, we design a
block-diagonal Cholesky preconditioner which leverages the structure of the data
matrix $\matQ$.

Recall from Appendix \ref{sec:data-matrix-definition} that
$\matQ$
takes the form of:
\begin{equation}
    \label{eq:matQ-full-form}
    \matQ = \begin{bNiceMatrix}
        L(G^{\rho}) + \Sigma & \zerosMat{\rotDim}{\distMeasureDim} & \tilde{V}\\
        \zerosMat{\distMeasureDim}{\rotDim} & W \tilde{D}^2 & C^\top W \tilde{D} \\
        \tilde{V}^\top & \tilde{D} W C & C^\top W C + L(G^{\tau}) \\
    \end{bNiceMatrix}.
\end{equation}

We leverage the block-structure of $\matQ$ to design a preconditioner.
Specifically, we strictly consider the block-diagonal approximation of $\matQ$,
\begin{equation}
    \tilde{\matQ} = \begin{bNiceMatrix}
        L(G^{\rho}) + \Sigma & 0 & 0 \\
        0 & W \tilde{D}^2 & 0 \\
        0 & 0 & C^\top W C + L(G^{\tau}) \\
    \end{bNiceMatrix}.
\end{equation}



This approximation has the advantage of being block-diagonal, which allows us to
compute the inverse of $\tilde{\matQ}$ by inverting each block separately.
Additionally, $\matQ$ is typically block-diagonally dominant due to graphical
structure of the problem \cite{rosen19ijrr,halsted22arxiv}, meaning that
$\tilde{\matQ}$ preserves much of the structure of $\matQ$. Furthermore, these
blocks are highly sparse, again due to the graphical structure of the problem.
This lends substantial computational efficiency to both the inversion of
$\tilde{\matQ}$ and application of the preconditioner.

To efficiently compute the inverse of the first block, $L(G^\rho) + \Sigma$, we
compute its Cholesky decomposition and use the resulting factorization to apply
the inverse. The second block, $W \tilde{D}^2$, is a diagonal matrix and thus
is trivially inverted.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/experiments/precon/cost_vs_iter_single_drone.png}
    \caption{\textbf{Solver cost over time:} the cost at a given iterate of the
        Rimannian Trust Region optimizer compared to the time spent in the optimizer
        up to that point.  The figure compares each preconditioner in the
        single-drone experiment (\cref{sec:drone-experiments}). The figure zooms in
        on the first 13 seconds to highlight the initial difference in convergence
        between the proposed block diagonal Cholesky preconditioner and the other
        preconditioners.
    }
    \label{fig:precon-cost-vs-iter}
    \vspace{-3mm}
\end{figure}

The third block, $C^\top W C + L(G^\tau)$, is notably the sum of two graph
Laplacians and thus is singular. This is due to the fact that graph Laplacians
have a nullspace which contains the all-ones vector. In our problem this
nullspace can be interpreted as the fact that the cost is identical up to a
translational offset, that is the estimated translations can be identically
shifted without incurring additional cost.

The existance of this nullspace means that the matrix $C^\top W C + L(G^\tau)$
is singular and thus cannot be inverted. However, we can `pin' the Laplacians
by removing a single row and corresponding column. This can be considered
equivalent to fixing the translational offset of the estimated trajectories
\cite{briales17ral}. Without loss of generality we choose to remove the last row
and column of $C^\top W C + L(G^\tau)$; from this point we can compute the
Cholesky decomposition of the resulting matrix and use the resulting
factorization to apply the inverse.

\def \pinnedLaplacian{\underline{L}_{tran}}
We denote the `pinned' matrix as $\pinnedLaplacian$. To account for the `pinned'
translational state when applying $\pinnedLaplacian^{-1} x$ as a preconditioner to
$x$ we ignore the last row of $x$ when applying $\pinnedLaplacian^{-1}$ and pad
the result with zeros. This corresponds to pinning the translational offset at
the origin.

We have established that our preconditioner $\matP$
consists of Cholesky decompositions of the first and third blocks of
$\tilde{\matQ}$ and the inverse of the second block of $\tilde{\matQ}$:
\begin{align}
     & R_r^\top R_r  = L(G^\rho) + \Sigma         \\
     & R_t^\top R_t  = \pinnedLaplacian           \\
     & \matP         = \begin{bNiceMatrix}
        (R_r^\top R_r)^{-1} & 0 & 0 \\
        0 & W^{-1} \tilde{D}^{-2} & 0 \\
        0 & 0 & (R_t^\top R_t)^{-1} \\
    \end{bNiceMatrix}.
\end{align}

We note that, for computational reasons, we never explicitly compute the
preconditioner $\matP$; the blocks of $\matP$ are generically dense and thus
expensive to store and apply. Instead, we store the Cholesky factors and apply
their inverses via forward- and back-substitution.

\subsection*{Evaluation}

We evaluate the performance of our preconditioner against the standard
preconditioners mentioned above: the Jacobi, block-Jacobi, incomplete Cholesky,
and regularized incomplete Cholesky preconditioners. As different
preconditioners may be cheaper to apply but result in slower convergence, we
evaluate the preconditioners in terms of the time spent in the Riemannian trust
region solver.

This is not the total time CORA spends solving each problem, as this neglects
the time spent in certification and saddle escape. This timing methodology
provides a clearer picture of the effect of the preconditioner on runtime.

We test each preconditioner on the real-world problems from
\cref{sec:real-world-evaluation} with identical parameters. All problems are
initialized with robot odometry, the first pose of each robot is given as ground
truth, and the positions of all landmarks are initialized at their ground truth
values.

We show the solver cost over time for the single-drone experiment in
\cref{fig:precon-cost-vs-iter}. It can be seen that the proposed block-diagonal
Cholesky preconditioner obtains a lower cost much more quickly than the other
preconditioners. The trends shown in \cref{fig:precon-cost-vs-iter} were
found to be consistent across all experiments.

The timing results for all experiments are shown in
\cref{tab:preconditioner-times}. For each experiment the block-diagonal Cholesky
preconditioner we designed for CORA obtains solutions 2-10 times faster than the
next fastest preconditioner.

\begin{table}[tbp]
    \centering
    \begin{tabularx}{0.95\linewidth}{ccccc}
        \toprule
        {Preconditioner}   & Single Drone    & Plaza 1         & Plaza 2        & TIERS           \\
        \midrule
        \textbf{Ours}      & \textbf{23 (s)} & \textbf{26 (s)} & \textbf{4 (s)} & \textbf{29 (s)} \\
        inc. Cholesky      & 44 (s)          & 76 (s)          & 14 (s)         & 229 (s)         \\
        block Jacobi       & 54 (s)          & 178 (s)         & 20 (s)         & 1468 (s)        \\
        Jacobi             & 54 (s)          & 207 (s)         & 41 (s)         & 927 (s)         \\
        reg. inc. Cholesky & 47 (s)          & 242 (s)         & 28 (s)         & 703 (s)         \\
        \bottomrule
    \end{tabularx}
    \caption{
        \textbf{Preconditioner performance:} the time spent in the Riemannian
        trust region solver for each preconditioner on all of the real-world
        experiments from \cref{sec:real-world-evaluation}.
    }
    \label{tab:preconditioner-times}
\end{table}


